A Theory of Available-by-Design Communicating Systems

Choreographic programming is a programming-language design approach that drives error-safe protocol development in distributed systems. Starting from a global specification (choreography) one can generate distributed implementations. The advantages of this top-down approach lie in the correctness-by-design principle, where implementations (endpoints) generated from a choreography behave according to the strict control flow described in the choreography, and do not deadlock. Motivated by challenging scenarios in Cyber-Physical Systems (CPS), we study how choreographic programming can cater for dynamic infrastructures where not all endpoints are always available. We introduce the Global Quality Calculus ($GC_q$), a variant of choreographic programming for the description of communication systems where some of the components involved in a communication might fail. GCq features novel operators for multiparty, partial and collective communications. This paper studies the nature of failure-aware communication: First, we introduce $GC_q$ syntax, semantics and examples of its use. The interplay between failures and collective communications in a choreography can lead to choreographies that cannot progress due to absence of resources. In our second contribution, we provide a type system that ensures that choreographies can be realized despite changing availability conditions. A specification in $GC_q$ guides the implementation of distributed endpoints when paired with global (session) types. Our third contribution provides an endpoint-projection based methodology for the generation of failure-aware distributed processes. We show the correctness of the projection, and that well-typed choreographies with availability considerations enjoy progress.

==> epc-types.tex <==
\subsection{Session Types for the End-Point Calculus}
\label{Logic4Struct-EndPointTypes}
Session types for the EPC use the syntax of session types in
equation \ref{Logic4Struct:eq:sessiontypes}. Basically, the type
discipline of the EPC stems from the Global Calculus, but assigns
session types to every single participant instead of the whole
choreography. In this way, the session typing in the EPC describes the
end-point behaviour.
% \begin{definition}[
% End-Point Typing Judgements
  An {\it end-point typing judgment} contains judgements for processes in  the form $\tprovesA{\Gamma}{P}{\Delta}$ (where $P$ is
    typed as a behaviour for $A$) and judgements for networks
    $\tproves{\Gamma}{N}{\Delta}$. In both,  mappings $\Gamma$ and $\Delta$ are {\em service} and {\em session typings} respectively.
%    triple on processes or
%   networks:\\
%   \begin{tabular}{ll}
%     (Processes) & $\tprovesA{\Gamma}{P}{\Delta}$ (where $P$ is
%     typed as a behaviour for $A$)\\
%     (Networks) & $\tproves{\Gamma}{N}{\Delta}$.  
%   \end{tabular}\\
%   where the mappings $\Gamma$ and $\Delta$ are the {\em service} and the {\em session typing} respectively.
% \end{definition}
Here, $\Gamma$ 
% (service typing)
 and $\Delta$ 
% (session typing) 
are defined
as:
\begin{align*}
&\Gamma  \ \; ::=\;\ \emptyset
                  \;\ |\;\ \Gamma, a@A\!:\!(\VEC{k})\alpha
                  \;\ |\;\ \Gamma, \ol{a}@A\!:\!(\VEC{k})\alpha
                  \;\ |\;\ \Gamma, x@A\!:\!\theta
                  \;\ |\;\ \Gamma, X\!:\!\Delta
%\qquad
\\
&\Delta  \ \; ::=\;\ \emptyset
              \;\ |\;\ \Delta, \VEC{k}@A\!:\!\alpha
              \;\ |\;\ \Delta, \VEC{k}\!:\!\bot
\end{align*}

Above, $a@A\!:\!(\VEC{k})\alpha$ indicates the service located at $A$
which is invoked with fresh session channels $\VEC{k}$ and offers
service of the shape $\alpha$, while $\ol{a}@A\!:\!(\VEC{k})\alpha$
indicates the type abstraction for the dual invocation, i.e. a client
of a service offered by $A$ which invokes with fresh channels $\VEC{k}$ and
engages in interactions abstracted as $\alpha$. Note $@A$ indicates
the location of a service in both forms. 
As before, $\VEC{k}$ should be a vector of pairwise distinct session
channels which should cover all session channels in $\alpha$, and
$\alpha$ does not contain free type variables. $(\VEC{k})$ binds
occurrences of session channels in $(\VEC{k})$ in $\alpha$, which
induces the standard alpha-equality. A central concept in this type
discipline is the notion of duality for session types, which is defined as:
\[
\ol{\!(\VEC{k})\alpha}@A = ? (\VEC{k}) \ol{\alpha}@A ~~~~~~
\ol{? (\VEC{k}) \alpha@A} = \! (\VEC{k}) \ol{\alpha}@A 
\]
where the notion of duality $\alpha$ of $\alpha$ remains the same.




The typing rules are almost identical as the ones from the original
presentation of the EPC \cite{carbone7scc}, where the only difference
lies on the separation between input-output types and
selection-branching types as originally presented in
\cite{honda1998lpa}. Here we only comment some examples on the typing
rules, and the full type system can be found in Appendix
\ref{Logic4Struct:appendix:EPC-Types}. As in our account of the type
system for the Global Calculus, we here devote our attention to the
rules for session initiation and communication.  The two rules
\Did{E-TInit.In},\Did{E-TInit.Out} describe session initiation
primitives:


\begin{align*}
  \inferenceg{ E-TInit.In} 
  { \typerule{\typeEnv }{A}{ P \ccc
      \VEC{k}@A:\alpha} 
    \quad a \not\in dom(\typeEnv) 
    \quad    client(\typeEnv) 
  } { 
    \typerule{\typeEnv, a @ A: (\VEC{k}) \alpha }{A}{
      !a(\VEC{k}) \pfx P \ccc \emptyset}
  }
  \quad 
  \inferenceg{ E-TInit.Out} 
  { \typerule{\typeEnv, a@B:(\VEC{k})\alpha}{A}{ P \ccc \Delta \cdot
      \VEC{k}@A:\alpha}  } 
  { \typerule{\typeEnv, a @B: (\VEC{k})\alpha }{A}{ \overline{a}
      <. \VEC{k} .> P \ccc \Delta}}
\end{align*}

In \Did{E-TInit.In}, the premise only allows for typings of session
channels involved in the session initialisation of service $a$, that
is,  only the channels in $\VEC{k}$. This linearity condition blocks
free session channels from occurring during a replicated input. The
condition $a \not\in dom(\typeEnv)$ prevents from self-calls and
ensures that the type assignment occurs at the side of the client.
Requirements for the complementary typing rule \Did{E-TInit.In} are
analogous, although the linearity condition is removed. Communication
rules are standard for session types, for instance, the rule
\Did{E.TOut} is used to type message outputs:

\begin{align*}
  \myrule{    E.TOut}
    { 
      k \in \VEC{k} \quad
      \typerule{\typeEnv  }{A}{ 
        P  \ccc \Delta \cdot \VEC{k}@A:\alpha} \quad 
      \typerule{\typeEnv  }{}{ e : \theta} 
    } 
    { \typerule{\typeEnv  }{A}{
        \send{k}{e}  P  \ccc \Delta
      \cdot \VEC{k}@A: k \uparrow \theta
    \pfx \alpha}}
\end{align*}

Here, process $\send{k} {e}  P$ types after evaluation that the typing
of $e$ corresponds to a correct value type and that the continuation
$P$ behaves as established by the session type  in $\Delta \cdot
\VEC{k}@A:\alpha$. Analogous requirements hold for typing the input
process $ \receive{k}{x}  P$.

% \begin{theorem}\label{theorem:epc:sr}\

%   \begin{enumerate}
    
%   \item (Subject Congruence) If $\tproves{\Gamma}{M}{\Delta}$ and
%     $M\LITEQ N$ then $\tproves{\Gamma}{N}{\Delta}$;

%   \item (Subject Reduction) If $\Gamma\vdash N\rhd\Delta$ and
%     $N\rightarrow N'$ then $\Gamma\vdash N'\rhd\Delta$.

%   \end{enumerate}

% \end{theorem}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> epp-types.tex <==
\subsection{End Point Projection}
\label{Logic4Struct:sec:epp-types}


The relation between global and local views at the specification of
communication protocols is given at the level of types. The central
idea is that one can \emph{project} the behaviour (type) of a
global specification given in terms of choreography into a parallel
composition of the behaviours of end-points. The mapping is far from
trivial, and needs to preserve causal relations between messages and
threads, namely \emph{connectedness}, \emph{well-threadedness} and
\emph{coherence}. The next subsection
presents a recap from the work at \cite{carbone7scc}. We will use
these definitions (specially Theorem \ref{Logic4Struct:theorem:epp}
and Definition \ref{Logic4Struct:definition:pruning}) in order to
relate the work on end-point projections with their corresponding
logical counterpart.
In order to give the formal definition of end point projection, we
first annotate global specifications with identifiers for threads.

% \begin{definition}[Annotated Interactions]
  An annotated interaction is an annotation of a choreography with
  $t$'s denoting each thread in play. Annotated interactions are
  written $\mathcal{A,A', ...}$, and they are given by
  the following grammar:

  \begin{align*} 
    \CAL{A} ::= & ~~~\initA{A^{t_1}}{ B ^{t_2}}{a}{k} \pfx \CAL{A}
    && |~~\CAL{A}_1 |^t \CAL{A}_2 \\
    & |~~\interactA{A^{t_1}}{ B ^{t_2}}{k}{e}{y} \pfx \CAL{A}
    && |~~\mu^t X^A \pfx \CAL{A}\\
    & |~~\choiceA{A^{t_1}}{B ^{t_2}}{k}{l}{\CAL{A}}
    && |~~ X^A_t \\
    & |~~\itn{e@A^{t}}{\CAL{A}_1}{\CAL{A}_2}
    && |~~\INACT
\end{align*}
where each $t$ is a natural number. We call $t,t',\cdots$ occurring in
an annotated interaction, \emph{threads}. Each $\CAL{A}$ can be
regarded as an abstract syntax built from a constructor in its root
(either a prefix or a parallel product), if the tree is originated
from a single thread, or a pair of threads if the interaction involves
an interaction (session initiation, message communication or
selection/branching). The following is the consistent annotation of
(\ref{Logic4Struct:example:syntax}).


\begin{align}
      & \initA{\text{Cust}^1}{\text{AC}^2}{\text{ob}}{k_1,k_2} \pfx
    \interactA{\text{Cust}^1}{\text{AC}^2}{k_1}{\text{booking}}{x} \pfx \tag{$OB_{\CAL{A}}$} \\
     & ~~~~~~\interactA{\text{AC}^2}{\text{Cust}^1}{k_2}{\text{offer}}{y} \pfx
    \interactA{\text{Cust}^1}{\text{AC}^2}{k_1}{\text{accept}}{z} \pfx
    \INACT \notag 
\end{align}

This annotation, though simple, would become more complicated if there
more than one session initiation was involved in the choreography.
 Take for instance the case where
$\initA{\text{Cust}}{\text{AC}}{\text{ob}}{k_1,k_2}$ is decomposed by
the sequence of processes
$\initA{\text{Cust}}{\text{AC}}{\text{ob}}{k_1}\pfx$ $
\initA{\text{AC}}{\text{Cust}}{\text{ob}}{k_2}$ We can have different
annotations for Cust and AC. The sequence:
$\initA{\text{Cust}^1}{\text{AC}^2}{\text{ob}}{k_1}\pfx
\initA{\text{AC}^2}{\text{Cust}^3}{\text{ob}}{k_2}$ generates a valid
annotation as it places each session initiation between the customer
and the AC in different threads, and any other annotation would be
invalid.
% \end{definition}


A choreography $\chor$ is \emph{connected}, if in communication
actions, only the message reception leads to activity (at the
receiving participant), and that such activity should immediately
follow the reception of messages. 
Informally, for each participant $A$ in the set of
participants of a choreography $\chor$, a communication activity
originated by $A$ should have been immediately preceeded by a communication
activity where $A$ had acted as a receiver, or been preceded by a
self-contained action (evaluation of expressions, for instance).

% With respect to threads, it is convenient to introduce some notation: $t_1$
%     (resp. $t_2$) is the \emph{active thread} of $\CAL{A}$ by $B$ (resp.
%     the \emph{passive thread} of $\CAL{B}$ by $C$) if the root of $\CAL{A}$
%     is initialisation/communication from 
%     $B$ to $C$ and it is annotated by $(t_1 , t_2 )$. We define
%     predecessors and successors in annotated interactions as normally
%     defined in ASTs: A direct predecessor is a predecessor which has no
%     intermediate predecessor. Symmetrically we define successor and
%     direct successor. 
% \begin{definition}[Threads]
%   \begin{enumerate}
%   \item If the root of $\CAL{A}$ is initialisation/communication from
%     $B$ to $C$ and is annotated by $(t_1 , t_2 )$, then $t_1$
%     (resp. $t_2$) is the active thread of $\CAL{A}$ by $B$ (resp.
%     the passive thread of $\CAL{B}$ by $C$). If the root of $\CAL{A}$ is
%     another constructor then its annotation $t$ is both its active
%     thread and its passive thread.
%   \item If $\CAL{A'}$ occurs as a proper subtree of $\CAL{A}$, then
%     (the root of) $\CAL{A}$ is a predecessor of (the root of)
%     $\CAL{A'}$. A direct predecessor is a predecessor which has no
%     intermediate predecessor. Symmetrically we define successor and
%     direct successor. 
% \end{enumerate}
% \end{definition}


\paragraph{Consistent annotations} In order to provide meaningful
projections between choreographies and its end-points, we need to
define a notion of ``consistent annotation'', that is, an annotation
$\CAL{A}$ such that it respects causality conditions, and can be
realised by a projection.
% \begin{definition}[Consistently Annotated Interactions] \label{Logic4Struct:def:cons-annotated-ints}
%   A well-typed annotated connected interaction (choreography)
%   $\mathcal{A}$ is consistent if the following conditions hold for
%   each of its subtrees, say $\mathcal{A'}$:
Such conditions are: 1) Causal Consistency: if a participant annotated
with $t$ is passive in an interaction (a receiver), then the
subsequent interaction will be marked with $t$ as well, or it will be
a self-contained action, 2) Session Consistency: Two actions in
$\CAL{A}$ identified by the same session name are annotated with the
same thread, and 3) Distinctness Condition: The input of session
initiation is always given a fresh thread.

%   \begin{itemize}
%   \item[--]Freshness Condition (FC):  If $t$ is by $\mathcal{A}$ at
%     some node and by $\mathcal{B}$ at another node then $\mathcal{A}$
%       and $\mathcal{B}$ always coincide. Further, if $\mathcal{A'}$
%       starts with an initialisation, then its passive thread should be
%       fresh w.r.t. all of its predecessors (if any).
%     \item[--]Session Consistency (SC): If $\mathcal{A'}$ starts with a
%       communication between $\mathcal{B}$ and $\mathcal{C}$ via (say)
%       $k$ and another subtree $\mathcal{A''}$ of $\mathcal{A}$ starts
%       with a communication via $k$ or an initialisation which opens
%       $k$, then the thread by $\mathcal{B}$ (resp. by $\mathcal{C}$)
%       of $\mathcal{A'}$ should be equal to the thread by $\mathcal{B}$
%       (resp. by $\mathcal{C}$) of $\mathcal{A''}$.
%     \item[--]Causal Consistency (CC): If $\mathcal{A''}$ is the direct
%       successor of $\mathcal{A'}$, then the active thread of
%       $\mathcal{A''}$ should coincide with the passive thread of
%       $\mathcal{A'}$.  We also say $\chor$ is well-threaded when there
%       is a well-formed annotation $\mathcal{A}$ of $\chor$ (i.e. the
%       result of erasing the annotations from $\mathcal{A}$ coincides
%       with $\chor$).
%     \end{itemize}
%     We also say $\chor$ is well-threaded when there is a well-formed annotation $\mathcal A$ of $\chor$ (i.e.: The result of erasing the annotations from $\mathcal A$ coincides with $\chor$).
% \end{definition}


The \emph{Well-threadedness} condition ensures global specifications
are free from unrealisable dependencies among actions. We say $\CAL{A}$
is well-threaded if it is connected and it has a consistent
annotation. 



% \begin{definition}[Mergeability]
\paragraph{Mergeability}
 Annotations in a choreography allow for the extraction of threads
 directly from the global behaviour. As threads are 
 sequences of actions to be executed at each end-point, we need to ensure that
 threads generated from choreographical annotations are meaningful, in
 the sense that they project only to the required end-points, and
 threads describing the behaviour of the same end point are
 encapsulated (\emph{merged})  on a single service description. 
  Mergeability, denoted by $\mergeable$, is the smallest equivalence
  over typed terms up to $\equiv$, closed under all typed contexts and

\begin{align*}
& \myruleg{M-Sel} 
   { 
	\forall i \in (J \cap H). (P_i \mergeable Q_i) \quad \forall j \in J\backslash H. \forall h \in H\backslash J. \mathsf{l}_j \neq \mathsf{l}_h
    }
    { \branching{k}{\Sigma_{j \in J} \mathsf{l_j} \pfx P_j}{}  \mergeable \branching{k}{\Sigma_{h \in H} \mathsf{l_h} \pfx P_h}{}
    } \quad 
%  \myruleg{M-In} 
%  { 
% 	x = y \quad P \mergeable Q
%  }
%  { \receive{k}{x} P \mergeable \receive{k}{y} Q   }
 \myruleg{M-Zero} 
 { 
	fsc(P) = 0
 }
 { P \mergeable \INACT   }
\end{align*}
When $P \mergeable Q$, we say that $P$ and $Q$ are mergeable.

% \end{definition}


Above, a context is any end-point calculus process with some
holes. $\Did{M-Sel}$ is for branching and says that we can allow
differences in branches which do not overlap, but we do demand each
pair of behaviours with the same operation to be identical.


The operation $P \merge Q$ allows for merging typed processes as long
as they are mergeable according to the rules above. $P \merge Q$ is a
partial commutative binary operator on typed processes which is
well-defined iff $P \mergeable Q$. We see an example of the merging
rules, and the full set can be consulted in Appendix
\ref{Logic4Struct:appendix:EPP-merging}. The merging of two branching
processes $\branching{k}{\Sigma_{i \in I} \mathsf{l_i} \pfx P_i} $
and $\branching{k}{\Sigma_{i \in J}}$ is given as:
\begin{align*}
	\branching{k}{\Sigma_{i \in I} \mathsf{l_i} \pfx P_i}{}\merge \branching{k}{\Sigma_{i \in J} \mathsf{l_i} \pfx Q_i}{} & \DEFEQ \branching{k}{ \begin{array}{l} \Sigma_{i \in I\cap J} \mathsf{l_i} \pfx P_i \merge Q_i \\ +\Sigma_{i \in I \backslash J} \mathsf{l_i} \pfx P_i  \\ +\Sigma_{i \in  J \backslash I} \mathsf{l_i} \pfx Q_i \end{array}  }{}
\end{align*}
That is, the resulting merge  groups in a single session branching all the
options coming from multiple branches that have the same session key.





Given a consistent annotation, we can project each of its threads onto
an end-point process. The thread
projection $\tp{\CAL{A}}{t}$ is a partial operation that uses the
merge operator, some of the rules are given below (the full set are
included in Appendix \ref{Logic4Struct:appendix:EPP-thread-proj}):


{\small
\[
\tp{\initA {A^{t_1}}{B^{t_2}}{b}{\tilde k}\pfx\mathcal A}{t}
    \DEFEQ
  \quad  \left\{ 
      \begin{array}{ll}
        \initOut{b}{\tilde k}\pfx\tp{\mathcal A}{t_1}
        &         
        \textrm{if}\ t=t_1\\
        \repInitIn{b}{\tilde k}\pfx\tp{\mathcal A}{t_2}
        & 
        \textrm{if}\ t=t_2\\
        \tp{\mathcal A}{t}
        & 
        \text{otherwise}
      \end{array}
    \right.
\]

\[\tp{\choice {A^{t_1}}{B^{t_2}}{k}{l}{\CAL{A}}}{t}
    \DEFEQ
    \quad\left\{ 
      \begin{array}{ll}
        \selection {k} {l_i}\tp{\mathcal A_i}{t}
       &                 \textrm{if}\ t=t_1
\\
        \branching k {\sum_i l_i}\pfx\tp{\mathcal A_i}{t}
        & 
        \textrm{if}\ t=t_2\\
        \tp{\mathcal A}{t}
        & 
        \text{otherwise}
      \end{array}
    \right.
\]

\[ \tp{\itn{e@A^{t'}}{\mathcal A_1}{\mathcal A_2}}{t}
    \DEFEQ
   \quad    \left\{ 
      \begin{array}{ll}
        \itn{e}{\tp{\mathcal A_1}{t'}}{\tp{\mathcal A_2}{t'}}
        &         
        \textrm{if}\ t=t'\\
        \tp{\mathcal A_1}{t}\merge\tp{\mathcal A_2}{t}
        & 
        \text{otherwise}
      \end{array}
    \right.
\]
}









\begin{definition}[Coherent Interactions]
  Given a well-threaded, consistently annotated interaction $\CAL{A}$,
  we say that $\CAL{A}$ is coherent if the following two conditions
  hold:
  \begin{enumerate}
    \item For each thread $t$ in $\CAL{A}$, $TP(\CAL{A},t)$ is
      well-defined. 
    \item For each pair of threads $t_1,t_2$ in $\CAL{A}$ with
        $t_1 \equiv_A t_2$, we have $TP(A,t_1) \mergeable
        TP(\CAL{A}, t_2)$. 
      \end{enumerate}
\end{definition}

Below, 
% we say $\chor$ is restriction-free whenever it contains no
% terms of the form $\new{a}\chor'$ as its subterm. Additionally, 
$part(\chor)$ denotes the set of participants names occurring in
$\chor$. Recall also being coherent entails being well-typed,
connected and well-threaded.


\begin{definition}[End-Point Projection]
\label{Logic4Struct:def:epp}
% Let $\chor$ be a coherent interaction such that $\chor\LITEQ \new {\tilde
%   s}\chor'$ where $\chor'$ is restriction-free. Let $\mathcal A$ be a
% consistent annotation of $\chor'$.  
Let $\chor$ be a coherent interaction, and %  such that $\chor\LITEQ \new {\tilde
%   s}\chor'$
%  where $\chor$ is restriction-free. 
 $\mathcal A$ be a
consistent annotation of $\chor$.  
% Then the {\em end point projection of
%   $\CAL{A}$ under a state $\sigma$}, denoted $\epp{\new{\tilde
%     s}\CAL{A}}{\sigma}$, is given as the following network.
Then the {\em end point projection of
  $\CAL{A}$ under a state $\sigma$}, denoted $\epp{\CAL{A}}{\sigma}$, is given as the following network.
\[
\epp{\CAL{A}}{\sigma} \DEFEQ
\Pi_{A \in part(\chor)}\ 
\pr
{A}
{\Pi_{[t]}\bigsqcup_{t'\in[t]}\tp{\mathcal A}{t'}}
{\sigma@A}
\]
\end{definition} 

The mapping given above is defined after choosing a specific
annotation of an interaction. The following result shows the map in
fact does not depend on a specific (consistent) annotation chosen, as
far as a global description has no incomplete threads, i.e. it has no
free session channels (which is what programmers/designers usually
produce).

\begin{theorem}[Soundness and Completeness of End-point Projections\cite{carbone7scc}]
  \label{Logic4Struct:theorem:epp}
  Assume $\mathcal A$ is well-typed, strongly connected, well-threaded
  and coherent. Assume further $\typerule{\typeEnv}{}{\mathcal A \ccc
    \Delta}$ and $\typerule{\typeEnv}{}{\sigma}$. Then the following
  properties hold: 

\begin{itemize}
  \item (soundness) if $\epp{\mathcal{A}}{\sigma}\action{}  \network$
    then there exists $\mathcal A'$ such that $(\sigma, \mathcal{A}) \action{}
(\sigma', \mathcal{A'})$ such that $\epp{\mathcal{A'}}{\sigma'} \prune \equiv_{rec} \network$.

 \item (completeness) If $(\sigma, \mathcal{A}) \action{}  (\sigma', \mathcal{A'})$ then there exist $\network$ such
   that $\epp{\mathcal{A}}{\sigma} \action{} \network$ and $\epp{\mathcal{A'}}{\sigma'} \prune \network$.

  \item (soundness with action labels) if $\epp{\mathcal{A}}{\sigma}\action{\emm}  \network$
    then there exists $\mathcal A'$ such that $(\sigma, \mathcal{A}) \action{\ell}
(\sigma', \mathcal{A'})$ such that $\epp{\mathcal{A'}}{\sigma'} \prune \equiv_{rec} \network$.

 \item (completeness with action labels) If $(\sigma, \mathcal{A}) \action{\ell}  (\sigma', \mathcal{A'})$ then there exist $\network$ such
   that $\epp{\mathcal{A}}{\sigma} \action{\emm} \network$ and $\epp{\mathcal{A'}}{\sigma'} \prune \network$.

\end{itemize}
\end{theorem}

Where $\equiv_{rec}$ denotes equality induced by the unfolding of
process recursion. The asymmetric relation $P \prune Q$ indicates that $P$ is the result
of cutting off ``unnecessary branches'' of $Q$, in the light of P's
own typing, is formally defined as follows:


\begin{definition}[Pruning]\label{Logic4Struct:definition:pruning}
 Let $\typeEnv |-_{A} P |> \Delta$ for $\typeEnv$ and $\Delta$
minimal and $\typeEnv, \typeEnv' |-_{A} Q |> \Delta$. If further we
have $Q \equiv Q_0 \pp !R$ where $\typeEnv |- Q_0 |> \Delta$, $\typeEnv'
|-_{A} R |> \Delta$ and $P \mergeable Q_0$, then we can write: $\typeEnv |-_A P \prune Q |>
\Delta$ or $P \prune Q$ for short, and say $P$
prunes $Q$ under $\typeEnv; \Delta$. $\prune$ is extended to networks accordingly.
\end{definition}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig-auxiliar-semantics.tex <==
\begin{figure}[t!]
% \hspace{\horizontalskip}
{\footnotesize
% \begin{subfigure}[b]{\linewidth}
%   \begin{gather*}
%     \qquad \quad 
%     \frac{ % Disjoint interactions
%       \threads{\chorAct} ~\#~       \threads{\chorAct'} 
%     }{
%       \chorAct;\chorAct' \swaps \chorAct' \pfx \chorAct
%     }
% \quad 
%     \frac{p \notin \threads{\chorAct}}{
%       \ifthenelsek {e@p} { \chorAct \pfx \chor_1}
%       { \chorAct \pfx \chor_2} \swaps
%       \chorAct \pfx\ifthenelsek {e@p} { \chor_1} { \chor_2} }
% \\
%     \frac{p \neq q}{
%       \ifthenelsek {e@p} {(\ifthenelsek {e'@q} {\chor_1} {\chor_2})}
%       {(\ifthenelsek {e'@q} {\chor'_1} {\chor'_2})} \swaps
%       \ifthenelsek {e'@q} {(\ifthenelsek {e@p} {\chor_1} {\chor'_1})} 
%       {(\ifthenelsek {e@p} {\chor_2} {\chor'_2})}}
%   \end{gather*}
%   \phantomsubcaption\label{fig:swap-rel}
%   % \caption{Swap congruence relation, $\swaps$}
% \end{subfigure}
\begin{subfigure}[b]{\linewidth}
  \begin{align*}
    % & \Rule{\chorAct = \bcastA{p_1}{p_2:x_2, \ldots,
    % p_j:x_j}{q}{e}{k} \quad \evalOp{e@p_1}{v} \quad \irange i2j } {
    % \effectOp kv\chorAct{\big(\bcastA{p_1}{p_2:x_2, \ldots,
    % p_i:\subst{v}{x_i}, \ldots, p_j:x_j}{q}{e}{k} \big)}} \quad
    % \Rule{\chorAct \neq \Did{Bcast}} { \effectOp
    % k{v}\chorAct\chorAct}
    % \\\\\hline\\
      & 
        \Rule{
        \begin{array}{c}
          \chorAct = \reduceA{\thread_1[A_1]\Blue{\{X_1;Y_1\}}.e_1,
          \ldots,
          \thread_j[A_j]\Blue{\{X_j;Y_j\}}.e_j}{\thread_{B}[B]\Blue{\{X_{B};Y_{B}\}}:x}{q}{k}{op}  
          ~~ 
          \evalOp{e_i@\thread_i}{v_i}
          \\
          \Blue{ X_i} \subseteq \sigma(\thread_i, k)
          \quad
          % \sigma'(\thread_i) =
          % \exchange{X_i}{Y_i}(\sigma(\thread_i))
          \sigma'= \update{(\thread_i, k)}{\exchange{\Blue{
          X_i}}{\Blue{ Y_i}}(\sigma(\thread_i,k))} 
          \quad
          \irange i1j      
        \end{array}
    } 
    {  
    \preduces{
    \conf{\sigma}{\chorAct \pfx \chor}
    }{(\thread_i,k) \colon \Blue{ X_i}::\Blue{ Y_i}}{
    \conf{\sigma'}{
    \begin{array}{r}
    \left(\reduceA{\thread_1[A_1]\Blue{\{X_1;Y_1\}}.e_1,
    \ldots,\thread_i[A_i]\Blue{\{Y_i;Y_i\}}.\some{v_i},    \ldots,
      \right. \\
    \left.  \thread_j[A_j]\Blue{\{X_j;Y_j\}}.e_j}{\thread_{B}[B]\Blue{\{X_B;Y_B\}}:x}{q}{k}{op}\right)
    \end{array}
    \pfx \chor } 
    } }
  % \\ & \qquad \qquad \qquad \qquad \qquad \qquad \qquad
  % \Rule{\chorAct \neq \Did{Reduce}} {
  % \preduces{\conf{\sigma}{\chorAct}}{\conf{\sigma}{\chorAct}} }
  \end{align*}
  % \caption{Effect rules}
  \phantomsubcaption\label{fig:effect:rules}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
  \begin{align*}
% & \Rule{}{     \enoughInputsOp {p:x}{\false}{\subst{ \none}{x}}{[ ~ ]} }
% \quad 
% \Rule{}{      \enoughInputsOp {p:\subst{v}{x}}{\true}{\subst{
%   \some{v}}{x}}{[ ~ ]}}
% \\ &
% \Rule{
%       \enoughInputsOp{sb_1}{t_1}{\theta_1}{\chi_1} 
%       ~~ \ldots ~~
%       \enoughInputsOp{sb_n}{t_n}{\theta_n}{\chi_n}
%       }{
%       \enoughInputsOp{\qualityBinder{sb_1, \ldots, sb_n}{q}}{q(t_1,
%       \ldots, t_n)}{\theta_1 \circ \ldots \circ \theta_n}{\chi_1
%      \circ \ldots \circ \chi_n}}\\ 
& 
\Rule{}{     \enoughOutputs {p.e}{\false}{[ ~ ]} }
\qquad
\Rule{}{      \enoughOutputs {p.\some{v}}{\true}{[(p,\some{v})]}}
\qquad
\Rule{
      \enoughOutputs{sc_1}{t_1}{\theta_1} 
      ~~ \ldots ~~
      \enoughOutputs{sc_n}{t_n}{\theta_n}
      }{
      \enoughOutputs{\qualityBinder{sc_1, \ldots, sc_n}{q}}{q(t_1,
      \ldots, t_n)}{\theta_1 \circ
  \ldots \circ \theta_n}}
  \end{align*}  
  % \caption{Rules for $\enoughOutputs \beta{\phi}{\theta}$}
  \phantomsubcaption\label{fig:enoughInputs}
\end{subfigure}
\caption{(\ref{fig:effect:rules}) effects, and (\ref{fig:enoughInputs}) binding testing rules}
}
\end{figure}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig-causality-types.tex <==
\begin{figure}[t]
{\footnotesize
  \begin{align*}
&\qquad \qquad 
\inferenceg{TGinit}
{ % \isIndex{a}{\serviceT GAB} \quad 
  %    \isType[\Gamma,\isInit{ \widetilde{\thread_p[A] },
  %    \widetilde{\thread_q\left(B\right)}, k}]{\chor}{\stypeEnv, k \colon G} 
  %    \quad \widetilde{\thread_q} \not\in \typeEnv
}
{ \isFType{ \initA{\widetilde{\thread_p[A]}}{ \widetilde{\thread_q[B]}}{a}{k} \pfx \chor } % {\stypeEnv}
  }
\\[0.2cm] &
\inferenceg{TGbcast}
  { % \begin{array}{l}
    %   \qquad 
    %   \isIndex[\typeEnv]{ \thread_1} { \ownerT{k}{A} } 
    %  \quad
    %  \isIndex[\typeEnv]{ \thread_i} { \ownerT {k}{B_i} } 
    %  \quad 
    %  \isIndex{e@\thread_1}{S}
    %  \\
    %  \isType[\typeEnv, x_2@\thread_2 \colon S, \ldots, x_j@\thread_j
    %  \colon S]{\chor}{\stypeEnv, k
    %  \colon G }
    %  \qquad 
    %   \irange i2j
    % \end{array}
        \typeEnv \vdash e@P_1 \equiv x_1@P_1
        \quad 
        \isFTypeEx{ 
        \typeEnv \otimes \left( \oplus_{|2\ldots j|} \left( x_1@\thread_1[A]
        --o \lencod{q} \left( \powerset_{\geq |\lencod{q}|} \left(
        x_2@\thread_2[B_2], \ldots x_j@\thread_j[B_j] \right) \right)
        \right) \right)
        }{\chor}
     }
  {\isFType{
    \left( \bcastA{\thread_1[A]}{\thread_2[B_2]:x_2, \ldots,
     \thread_j[B_j]:x_j}{q}{e}{k} \right) \pfx \chor }% {\stypeEnv, k \colon \left(
     % \bcastT{A}{\VEC B}{S} \pfx G \right) }
        } 
\\[0.2cm] & 
\inferenceg{TGred}
  {
        \typeEnv \vdash e_i@P_i \equiv x_i@P_i 
             \quad
        \isFTypeEx{ 
        \typeEnv \otimes \left( \oplus_{ S_i \in \powerset_{\geq
     |\lencod{q}|} (\thread_1[A], \ldots, \thread_j[A_j]) } \left( \precedes{S_i}{x@B}
        \right) \right)   
        }{\chor}
     \quad \irange i1j
    % \begin{array}{l}
    %   \isIndex[\typeEnv]{ \thread_i} { \ownerT{k}{A_i} } 
    %  \quad
    %  \isIndex[\typeEnv]{ \thread_{j+1}} { \ownerT{k}{B} } 
    %  \quad 
    %  \isIndex{e_i@\thread_i}{S}
    %  \\
    %   \quad
    %   \isType[\typeEnv, x@t_{j+1} \colon S]{\chor}{\stypeEnv, k
    %   \colon G }     
    %   \qquad 
    %   \irange i1j
    % \end{array}
     } 
  {\isFType{\left( \reduceA{\thread_1[A_1].e_1, \ldots,
    \thread_j[A_j].e_j}{\thread_{j+1}[B]:x}{q}{k}{op} \right) \pfx \chor }% {\stypeEnv, k \colon
 % \left(     \bcastT{\VEC A}{B}{S} \pfx G\right) }
        } 
\\[0.2cm] &
\inferenceg{TGsel}
  {
        \isFTypeEx{ 
        \typeEnv \otimes \left( \oplus_{|2\ldots j|} \left( x_1@\thread_1[A]
        --o \lencod{q} \left( \powerset_{\geq |\lencod{q}|} \left(
        x_2@\thread_2[B_2], \ldots x_j@\thread_j[B_j] \right) \right)
     \right) \right)
    % \isIndex[\typeEnv]{ \thread_1} { \ownerT{k}{A} } 
    %  \quad
    %  \isIndex[\typeEnv]{ \thread_2} { \ownerT{k}{B_2} } 
    %  \quad \ldots \quad
    %  \isIndex[\typeEnv]{ \thread_j} { \ownerT{k}{B_j} } 
    %  \quad 
    %  \isType{\chor}{\stypeEnv, k
    %  \colon G_h }
    %  \quad
    %  h \in I
     }{\chor}
     } 
  {\isFType{ \left( \choiceA{\thread_1[A]}{\thread_2[B_2], \ldots,
     \thread_j[B_j]}{q}{k}{l_h} \right)
     \pfx \chor}% {\stypeEnv, k \colon \branchT A{\VEC B}lG}
     } \\
    & \qquad \qquad 
      \inferenceg{TGcomp}
      { 
      % \isType[\typeEnv, \kappa : \killT ]{P}{\stypeEnv} 
      % \quad 
      % \isType[\typeEnv, \kappa : \killT ]{Q
      % }{\stypeEnv >> \stypeEnv'} 
      % \quad 
      % \trueProp{t \ge 0} 
      } 
      {\isFType{\comp P{Q}t\killAct}% {\stypeEnv';\stypeEnv''}
      } 
    \\
    & \qquad
%       \inferenceg{TGseq}
%       {\isType{ \chorAct }{\stypeEnv_1} 
%       \quad 
%       \isType{ \chor }{\stypeEnv_2} 
%       \quad 
%       \stypeEnv_1 \# \stypeEnv_2} 
%       {\isType{ \chorAct \pfx \chor }{\stypeEnv_1 , \stypeEnv_2}} 
% \quad
      \inferenceg{TGsum}
      { 
      \isFType{\chor}\quad \isFTypeEx{\typeEnv'}{\chor'}
      % \isType{ \chor }{\stypeEnv} \quad \isType{ \chor' }{\stypeEnv} 
      } 
      {\isFTypeEx{\typeEnv \oplus \typeEnv'}{ \chor + \chor'}% {\stypeEnv}
      } 
\quad
\inferenceg{TGres}
  { 
      % \isType[\Gamma, r:S]{ \chor}{\stypeEnv}
      \isFType{\new{r} \chor} 
      \quad 
      r \in \fv{\typeEnv} \setminus \fv{\chor}
      } 
  {\isFTypeEx{\exists r. \typeEnv}{ \chor}% {\stypeEnv}
      } 
\quad
\inferenceg{TGinact}
  { % \isEnd
      } 
  {\isFTypeEx{\endT}{ \INACT }% {\stypeEnv}
      } 
\\& \qquad \qquad 
\inferenceg{TGcond}
  { 
    \isFType{\chor_1}
    \quad
    \isFType{\chor_2}
    % \isType{\chor_1}{\stypeEnv} 
    % \quad
    % \isType{\chor_2}{\stypeEnv} 
    % \quad 
    % \isProp{e@\thread} 
    } 
  {\isFType{ \ifthenelsek {e@\thread} {\chor_1} {\chor_2} }% {\stypeEnv}
    } 
\quad
\inferenceg{TGkill}
  {
    % \isIndex{\kappa}{\killT}
    } 
  {\isFType{ \killOp{\kappa}}% {\stypeEnv}
    } 
\\& \qquad \qquad 
\inferenceg{TGrec}
  { 
    % \begin{array}{l}
    %   \isType[\typeEnv, X(\VEC D) \colon
    %   (\typeEnv';\stypeEnv')]{\chor}{\stypeEnv}
    %   \quad
    %   \isType[\typeEnv', X(\VEC D) \colon
    %   (\typeEnv';\stypeEnv')]{\chor'}{\stypeEnv'}
    %   \\ \qquad 
    %   \widetilde D = p_1(\VEC{x_1}, \VEC{k_1}), \ldots, p_n(\VEC{x_n},
    %   \VEC{k_n})
    %   \quad
    %   \isShared[\typeEnv'] \subseteq \typeEnv
    % \end{array}
    } 
  {\isFType{ \recA{X}{\VEC{D}}{\chor'}{\chor} }% {\stypeEnv}
        } 
\\& \qquad \qquad \quad
\inferenceg{TGcall}
  { 
    % \begin{array}{l}
    %   \quad
    % \isEnd
    % \quad
    % \isType[\typeEnv'']{x_{ij}@p_i}{S_{ij}}
    % \quad
    % \isType[\typeEnv]{e_{ij}@p_i}{S_{ij}}
    % \quad
    % \typeEnv'\subseteq \typeEnv
    % \\
    % \widetilde D = p_1(\VEC{x_1}, \VEC{k_1}), \ldots, p_n(\VEC{x_n}, \VEC{k_n})
    % \quad
    % \widetilde E = p_1(\VEC{e_1}, \VEC{k_1}), \ldots, p_n(\VEC{e_n}, \VEC{k_n})
    % \end{array}
    } 
  {\isFType[\typeEnv, X(\widetilde D) \colon (\typeEnv',\typeEnv'' ;
         \stypeEnv')]{ X(\VEC{E}) }% {\stypeEnv}
        } 
% \\ &
% \inferenceg{TGstruct}
%   {
%   \chor \action{\killOp{\killAct}} \chor'
%   \quad
%   \killAct \neq \gamma
%   }  {\comp{\chor}{\chor''}{t}{\gamma} \action{\killOp{\killAct}}
%   \comp{\chor'}{\chor''}{t}{\gamma}} 
  \end{align*}
}
  \caption{\GCQ: Type checking - Global types}
  \label{fig:global:types}
\end{figure}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig-effect-rules-epc.tex <==
\begin{figure}[t]
{\footnotesize
  \begin{align*}
%     & 
%      \Rule{\chorAct = \bcastA{p_1}{p_2:x_2, \ldots,
%       p_j:x_j}{q}{e}{k} 
%       \quad 
%       \evalOp{e@p_1}{v}
%       \quad
%       \irange i2j     } 
%       {  \effectOp kv\chorAct{\big(\bcastA{p_1}{p_2:x_2, \ldots,
%       p_i:\subst{v}{x_i}, \ldots, 
%       p_j:x_j}{q}{e}{k} \big)}} 
% \quad 
%       \Rule{\chorAct \neq \Did{Bcast}} 
%       {  \effectOp k{v}\chorAct\chorAct} 
% \\\\\hline\\
    & 
        \Rule{
        \begin{array}{c}
          \chorAct = \reduceA{\thread_1[A_1]\Blue{\{X_1;Y_1\}}.e_1,
          \ldots,
          \thread_j[A_j]\Blue{\{X_j;Y_j\}}.e_j}{\thread_{B}[B]\Blue{\{X_{B};Y_{B}\}}:x}{q}{k}{op}  
          ~~ 
          \evalOp{e_i@\thread_i}{v_i}
          \\
          \Blue{ X_i} \in \sigma(\thread_i, k)
          \quad
          % \sigma'(\thread_i) =
          % \exchange{X_i}{Y_i}(\sigma(\thread_i))
          \sigma'= \update{(\thread_i, k)}{\exchange{\Blue{
          X_i}}{\Blue{ Y_i}}(\sigma(\thread_i,k))} 
          \quad
          \irange i1j      
        \end{array}
    } 
    {  
    \preduces{
    \conf{\sigma}{\chorAct \pfx \chor}
    }{(\thread_i,k) \colon \Blue{ X_i}::\Blue{ Y_i}}{
    \conf{\sigma'}{
    \begin{array}{r}
    \left(\reduceA{\thread_1[A_1]\Blue{\{X_1;Y_1\}}.e_1,
    \ldots,\thread_i[A_i]\Blue{\{Y_i;Y_i\}}.\some{v_i},    \ldots,
      \right. \\
    \left.  \thread_j[A_j]\Blue{\{X_j;Y_j\}}.e_j}{\thread_{B}[B]\Blue{\{X_B;Y_B\}}:x}{q}{k}{op}\right)
    \end{array}
    \pfx \chor } 
    } }
  \end{align*}
  \caption{\EPQ: Effect rules.}
  \label{fig:effect:rules-epc}
}
\end{figure}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig-effect-rules.tex <==
\begin{figure*}[t!]
{\footnotesize
  \begin{align*}
%     & 
%      \Rule{\chorAct = \bcastA{p_1}{p_2:x_2, \ldots,
%       p_j:x_j}{q}{e}{k} 
%       \quad 
%       \evalOp{e@p_1}{v}
%       \quad
%       \irange i2j     } 
%       {  \effectOp kv\chorAct{\big(\bcastA{p_1}{p_2:x_2, \ldots,
%       p_i:\subst{v}{x_i}, \ldots, 
%       p_j:x_j}{q}{e}{k} \big)}} 
% \quad 
%       \Rule{\chorAct \neq \Did{Bcast}} 
%       {  \effectOp k{v}\chorAct\chorAct} 
% \\\\\hline\\
    & 
        \Rule{
        \begin{array}{c}
          \chorAct = \reduceA{\thread_1[A_1]\Blue{\{X_1;Y_1\}}.e_1,
          \ldots,
          \thread_j[A_j]\Blue{\{X_j;Y_j\}}.e_j}{\thread_{B}[B]\Blue{\{X_{B};Y_{B}\}}:x}{q}{k}{op}  
          ~~ 
          \evalOp{e_i@\thread_i}{v_i}
          \\
          \Blue{ X_i} \in \sigma(\thread_i, k)
          \quad
          % \sigma'(\thread_i) =
          % \exchange{X_i}{Y_i}(\sigma(\thread_i))
          \sigma'= \update{(\thread_i, k)}{\exchange{\Blue{
          X_i}}{\Blue{ Y_i}}(\sigma(\thread_i,k))} 
          \quad
          \irange i1j      
        \end{array}
    } 
    {  
    \preduces{
    \conf{\sigma}{\chorAct \pfx \chor}
    }{(\thread_i,k) \colon \Blue{ X_i}::\Blue{ Y_i}}{
    \conf{\sigma'}{
    \begin{array}{r}
    \left(\reduceA{\thread_1[A_1]\Blue{\{X_1;Y_1\}}.e_1,
    \ldots,\thread_i[A_i]\Blue{\{Y_i;Y_i\}}.\some{v_i},    \ldots,
      \right. 
    \left.  \thread_j[A_j]\Blue{\{X_j;Y_j\}}.e_j}{\thread_{B}[B]\Blue{\{X_B;Y_B\}}:x}{q}{k}{op}\right)
    \end{array}
    \pfx \chor } 
    } }
  \end{align*}
  \caption{Effects}
  \label{fig:effect:rules}
}
\end{figure*}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig-enough-Inputs.tex <==
\begin{figure}[t]
{\footnotesize
  \begin{align*}
% & \Rule{}{     \enoughInputsOp {p:x}{\false}{\subst{ \none}{x}}{[ ~ ]} }
% \quad 
% \Rule{}{      \enoughInputsOp {p:\subst{v}{x}}{\true}{\subst{
%   \some{v}}{x}}{[ ~ ]}}
% \\ &
% \Rule{
%       \enoughInputsOp{sb_1}{t_1}{\theta_1}{\chi_1} 
%       ~~ \ldots ~~
%       \enoughInputsOp{sb_n}{t_n}{\theta_n}{\chi_n}
%       }{
%       \enoughInputsOp{\qualityBinder{sb_1, \ldots, sb_n}{q}}{q(t_1,
%       \ldots, t_n)}{\theta_1 \circ \ldots \circ \theta_n}{\chi_1
%      \circ \ldots \circ \chi_n}}\\ 
& 
\Rule{}{     \enoughOutputs {p.e}{\false}{[ ~ ]} }
\quad
\Rule{}{      \enoughOutputs {p.\some{v}}{\true}{[(p,\some{v})]}}
\\ &
\Rule{
      \enoughOutputs{sc_1}{t_1}{\theta_1} 
      ~~ \ldots ~~
      \enoughOutputs{sc_n}{t_n}{\theta_n}
      }{
      \enoughOutputs{\qualityBinder{sc_1, \ldots, sc_n}{q}}{q(t_1,
      \ldots, t_n)}{\theta_1 \circ
  \ldots \circ \theta_n}}
  \end{align*}  
}
  \caption{Rules for $\enoughOutputs \beta{\phi}{\theta}$}
  \label{fig:enoughInputs}
\end{figure}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig-global-causality-logic-selected.tex <==
\begin{figure*}[t] {\footnotesize 
    \begin{align*}
      & \text{Choregraphy Formation }    (\isEntailed{ \chor}), \\
      & \qquad \qquad \quad \qquad \qquad 
        \inferenceg{Tinit} {
        \begin{array}{c} 
          \isEntailed[\ltypeEnv, \isInit{
          \VEC{\thread_r[A_r]\Blue{\{Y_r\}}}, \VEC{\thread_s[B_s]\Blue{\{Y_s\}}},
          k}]{\chor}
          \quad
          \{\VEC{\thread_s},k\} ~\#~ (\threads{\ltypeEnv} \cup
          \keys{\ltypeEnv}) 
        \end{array}
      }
      { 
        \isEntailed{ \initA{\widetilde{\thread_r[A_r]\Blue{\{Y_r\}}}}{
      \VEC{\thread_s[B_s]\Blue{\{Y_s\}}}}{a}{k} \pfx \chor } 
      } 
      % \quad
      % \inferenceg{Tres}
      % {
      % % \isType[\Gamma, r:S]{\psi}{ \chor}{\stypeEnv}
      % % \isEntailed[\psi]{ \chor\subst{r}{r'}}
      % \isEntailed[\ltypeEnv]{ \chor}
      % \quad
      % r \notin (\keys{\ltypeEnv} \cup \threads{\ltypeEnv})
      % }
      %   {
      % %   \isType[\Gamma]{\psi}{ \new{r} \chor}{\stypeEnv}
      %   \isEntailed[\ltypeEnv]{ \new{r} \chor}
      % }
      %   \qquad \quad \inferenceg{TGkill} { \isIndex{\kappa}{\killT}}
      %   {\isType{\psi}{ \killOp{\kappa}}{\stypeEnv}}
      \\[\ruleskip] &
                      \hspace{\horizontalskip}
                      \inferenceg{Tbcast}
                    { \begin{array}{c}
                        \forall^{\ge 1} J.\ s.t. \left(
                        \begin{array}{c}
                          J \subseteq \VEC{\thread_r}
                          ~\land~
                          q(J) 
                          ~\land~
                          \ltypeEnv = \psi_A, (\psi_j)_{j \in
                          J},  \ltypeEnv' 
                          % \\[\ruleskip] 
                          \quad 
                          % ~\land~
                          % \phi = \thread_A \colon
                          % \ownerTP{k}{A}{X_A} \bigotimes_{j \in J}
                          % (\thread_j \colon
                          % \ownerTP{k}{B_j}{X_j} )
                          % ~\land~
                          % \phi' = \thread_A \colon
                          % \ownerTP{k}{A}{Y_A} \bigotimes_{j \in J}
                          % \left( \thread_j \colon
                          %   \ownerTP{k}{B_j}{Y_j} \right)
                          ~\land~
                          \typerule
                          {
                          \psi_A, (\psi_j)_{j \in
                          J}
                        % ,\phi \lolli \phi'
                          }{}{
                            % \phi
                          \thread_A \colon
                          \ownerTP{k}{A}{X_A} \bigotimes_{j \in J} (\thread_j \colon
                          \ownerTP{k}{B_j}{X_j}  ) 
                          } 
                        \end{array}
                        \right):
                        \\
                        % \typerule
                        % {
                        % \left(
                        %   \bigoplus_{i \in \{1, \ldots, m\}}
                        %   \psi^R_i
                        %   \oplus \left(
                        %     \thread_A \colon
                        %     \ownerTP{k}{A}{X_A} \bigotimes_{j \in J}
                        %     \left( \thread_j \colon
                        %       \ownerTP{k}{B_j}{X_j} \right)
                        %   \right)
                        %   \lolli
                        %   \left(
                        %     \thread_A \colon
                        %     \ownerTP{k}{A}{Y_A} \bigotimes_{j \in J}
                        %     \left( \thread_j \colon
                        %       \ownerTP{k}{B_j}{Y_j} \right)
                        %   \right)
                        % \right)
                        % }{}{
                        %   \thread_A \colon
                        %   \ownerTP{k}{A}{Y_A} \bigotimes_{j \in J}
                        %   \left( \thread_j \colon
                        %     \ownerTP{k}{B_j}{Y_j} \right)
                        % }
                        \isEntailed[      \thread_A \colon
                        \ownerTP{k}{A}{Y_A},  \left(\thread_j 
                        \colon \ownerTP{k}{B_j}{Y_j} \right)_{j \in
                        J},
                        \ltypeEnv']{\chor} 
                        \quad
                        \isOptData[e@\thread_A]
                        \quad
                        (\isOptData[x_i@\thread_i]) _{i =1}^{|\VEC{\thread_r}|}
                        % \isEntailed[\bigoplus_{i \in \{1, \ldots, m
                        % \}} \left(\psi^L_i
                        %   \otimes \thread_A \colon
                        %   \ownerTP{k}{A}{Y_A}
                        %   \bigotimes_{j \in J} \left( \thread_j
                        %     \colon \ownerTP{k}{B_j}{Y_j} \right)
                        % \right) ]{\chor}
                        % \psi = \psi' , \psi''
                        % \quad
                        % \isType[\typeEnv, \VEC{x_p@\thread_p[B_p]}
                        % \colon S]{\psi''
                        % , \psi'''}{\chor}{\stypeEnv, k
                        % \colon G }
                        % \quad
                        % \typerule{\psi' ,\thread_1 \colon
                        % \ownerT{k}{A} \lolli \psi'''}{}{\psi'''}
                        % \quad
                        % \notEntails{\ownerT{k}{A} \lolli \psi'}
                        % \quad
                        % \typerule{\psi,\psi'}{}{\chor}
                        % \quad
                        % \psi''' =\left(
                        %   \bigoplus_{J =
                        %   min(q(\widetilde{\thread_p[B_p]})) }
                        %   \left(
                        %     \bigotimes_{\thread_i \in J} (\thread_i
                        %     : \ownerT{k}{B_i})\right)\right)
                        % \quad
                        % t_i \in {\widetilde{t_p[B_p]}}
                      \end{array}
    }
    {
      % \isType{\psi}{
      % \left(
      %   \bcastA{\thread_1[A]}{\VEC{\thread_p[B_p]:x_p}}{q}{e}{k}
      % \right) \pfx \chor }{\stypeEnv, k \colon \left(
      %   \bcastT{A}{\VEC B}{S} \pfx G \right) }
    \isEntailed{
    \left( \bcastA{\thread_A[A]\Blue{\{X_A;Y_A\}}}{\VEC{\thread_r[B_r]\Blue{\{X_r;Y_r\}}:x_r}}{q}{e}{k} \right) \pfx \chor }
    } 
    \\[\ruleskip] &
                    \hspace{\horizontalskip}                    
                    \inferenceg{Tred}
                    { \begin{array}{c}
                        \forall^{\ge 1} J.\ s.t. \left( 
                        \begin{array}{c}
                          J \subseteq \VEC{\thread_r}
                          ~\land~ 
                          q(J)
                        ~\land~
                          \ltypeEnv = \psi_B, (\psi_j)_{j =1}^{|J|},
                          \ltypeEnv' 
                          \quad 
                          % \\
                        % ~\land~
                          % \phi =\thread_B \colon
                          % \ownerTP{k}{B}{X_B} \bigotimes_{j \in J} (\thread_j \colon
                          % \ownerTP{k}{A_j}{X_j}  ) 
                        % \ltypeEnv = (\psi_1^L \otimes \psi_1^R)
                        % \oplus \ldots \oplus
                        % (\psi_m^L \otimes \psi_m^R)
                          % \\ 
                          % ~\land~
                          % \phi' = \thread_B \colon
                          % \ownerTP{k}{B}{Y_B}      \bigotimes_{j \in J} \left( \thread_j \colon
                          % \ownerTP{k}{A_j}{Y_j} \right) 
                          ~\land~
                          \typerule
                          {
                          \psi_B,  (\psi_j)_{j =1}^{|J|}
                          % , \phi \lolli \phi'
                          }{}{
                          % \phi
                          \thread_B \colon
                          \ownerTP{k}{B}{X_B} \bigotimes_{j \in J} (\thread_j \colon
                          \ownerTP{k}{A_j}{X_j}  ) 
                          } 
                        \end{array}
                        \right): 
                        \\[\ruleskip]
                        \isEntailed[
                        \thread_B \colon  \ownerTP{k}{B}{Y_B},
                        \left(\thread_j \colon \ownerTP{k}{A_j}{Y_j}
                        \right) _{j =1}^{|J|}, 
                        \ltypeEnv']{\chor}
                        \quad
                        (\isOptData[e_i@\thread_i])_{i =1}^{|\VEC{\thread_r}|}
                        \quad
                        \isOptData[x@\thread_B]
                      \end{array}
    } 
    {
      % \isType{\psi,\psi''}{\left(
      %   \reduceA{\VEC{\thread_p[A_p].e_p}}{\thread[B]:x}{q}{k}{op}
      % \right) \pfx \chor }{\stypeEnv, k \colon
      % \left( \bcastT{\VEC A}{B}{S} \pfx G\right) }
    \isEntailed[\ltypeEnv]{\left(
    \reduceA{\VEC{\thread_r[A_r]\Blue{\{X_r;Y_r\}}.e_r}}{\thread_B[B]\Blue{\{X_B;Y_B\}}:x}{q}{k}{op}
    \right) \pfx \chor }
    } 
    \\[\ruleskip] & 
                    \inferenceg{Tsel}
                    { ((\text{as in \Did{Tbcast}}^*))
                      % \begin{array}{c}
                      %   \ltypeEnv = (\psi_1^L \otimes \psi_1^R)
    %    \oplus \ldots \oplus
    %   (\psi_m^L \otimes \psi_m^R) 
    %   \quad 
    %   J \subseteq \widetilde{B}
    %   \quad 
    %   q(J)
    %   \\
    %   \typerule
    %   {
    %   \bigoplus_{i \in \{1, \ldots, m\}} \psi^R_i 
    %   \oplus \left(
    %   \thread_A \colon
    %   \ownerTP{k}{A}{X_A} \bigotimes_{j \in J} \left( \thread_j \colon
    %   \ownerTP{k}{B_j}{X_j}  \right)
    %   \lolli 
    %   \thread_A \colon
    %   \ownerTP{k}{A}{Y_A} \bigotimes_{j \in J} \left( \thread_j \colon
    %   \ownerTP{k}{B_j}{Y_j} \right)
    %   \right)
    %   }{}{
    %   \thread_A \colon
    %   \ownerTP{k}{A}{Y_A} \bigotimes_{j \in J} \left( \thread_j \colon
    %   \ownerTP{k}{B_j}{Y_j} \right)     
    %   }
    %   \\
    %   \isEntailed[\bigoplus_{i \in \{1, \ldots, m \}} \left(\psi^L_i
    %   \otimes \thread_A \colon       \ownerTP{k}{A}{Y_A}
    %   \bigotimes_{j \in J} \left( \thread_j \colon
    %   \ownerTP{k}{B_j}{Y_j}  \right)   \right) ]{\chor}
    %   % \quad
    %   % t_i \in {\widetilde{t_p[B_p]}}
    % \end{array}
     } 
                {
                % \isType{\psi,\psi''}{ \left(
                % \choiceA{\thread_1[A]}{\widetilde{\thread_p[B_p]}}{q}{k}{l_h} \right)                % \pfx \chor}{\stypeEnv, k \colon \branchT A{\VEC B}lG} 
                \isEntailed[\ltypeEnv]{ \left( \choiceA{\thread_A[A]\Blue{\{X_A;Y_A\}}}{\VEC{\thread_r[B_r]\Blue{\{X_r;Y_r\}}}}{q}{k}{l_h} \right)                \pfx \chor}
                } 
    % \\[\ruleskip] & 
    % \qquad \qquad
                    \quad 
  \inferenceg{Tcond}
  { 
    % \isType{\psi}{\chor_1}{\stypeEnv} 
    % \quad
    % \isType{\psi}{\chor_2}{\stypeEnv} 
    % \quad
    % \isProp{e@\thread} 
  \isEntailed[\ltypeEnv]{\chor_1}
  \quad
  \isEntailed[\ltypeEnv]{\chor_2} 
  % \quad
  % \isProp{e@\thread} 
  }  
  {
    % \isType{\psi}{ \ifthenelsek {e@\thread} {\chor_1}
    % {\chor_2}    }{\stypeEnv}
  \isEntailed[\ltypeEnv]{ \ifthenelsek {e@\thread} {\chor_1}
  {\chor_2}    }
  } 
\\ &
  \inferenceg{Tinact}
                    { 
    % \isEnd
    % \quad\isSat\quad
                    \qquad 
                    } 
                    {
    % \isType{\psi}{ \INACT }{\stypeEnv}
                    \isEntailed[\ltypeEnv]{ \INACT }
                    } 
\qquad \qquad 
                    \inferenceg{Tsum}
                    { 
                      % \isType{\psi}{ \chor }{\stypeEnv} 
                      % \quad 
                      % \isType{\psi'}{ \chor' }{\stypeEnv} } 
                      \ltypeEnv = \psi \oplus \psi'
                      \quad 
                      \isEntailed[\psi]{ \chor }
                      \quad 
                      \isEntailed[\psi']{ \chor' }
                      } 
                      {
                        % \isType{\psi \oplus \psi'}{ \chor +
                        % \chor'}{\stypeEnv}
                      \isEntailed[\ltypeEnv]{ \chor + \chor'}
                      }  
                      % \\[\ruleskip]
                      % & \qquad \qquad \qquad \qquad
                      % \inferenceg{TGcomp}
                      % {
                      % \isType[\typeEnv, \kappa : \killT
                      %     %  ]{\psi}{P}{\stypeEnv}
                      %                 % \quad
                      %                 % \isType[\typeEnv, \kappa : \killT ]{\psi}{Q
                      %                 % }{\stypeEnv >> \stypeEnv'} 
                      %   %   \quad
                      %   %   \trueProp{t \ge 0}
                      % }
                      %   {\isType{\psi}{\comp
                %  P{Q}{}\killAct}{\stypeEnv';\stypeEnv''}}
                %   \\
% & 
% % \inferenceg{TGseq}
% % {\isType{\psi}{ \chorAct }{\stypeEnv_1} 
% % \quad 
% % \isType{\psi}{ \chor }{\stypeEnv_2} 
% % \quad 
% % \stypeEnv_1 \# \stypeEnv_2} 
% % {\isType{\psi}{ \chorAct \pfx \chor }{\stypeEnv_1 , \stypeEnv_2}} 
% % \\[\ruleskip] & 
% \inferenceg{Trec}
%   { \begin{array}{l}
%       \isType[\typeEnv, X(\VEC D) \colon
%       (\typeEnv';\stypeEnv')]{\psi}{\chor}{\stypeEnv}
%       \quad
%       \isType[\typeEnv', X(\VEC D) \colon
%       (\typeEnv';\stypeEnv')]{\psi}{\chor'}{\stypeEnv'}
%       \\ \qquad 
%       \widetilde D = p_1(\VEC{x_1}, \VEC{k_1}), \ldots, p_n(\VEC{x_n},
%       \VEC{k_n})
%       \quad
%       \isShared[\typeEnv'] \subseteq \typeEnv
%     \end{array}
%     } 
%   {\isType{\psi}{ \recA{X}{\VEC{D}}{\chor'}{\chor} }{\stypeEnv}} 
% \quad 
% \inferenceg{Tcall}
%   { 
%     \begin{array}{l}
%       \quad
%     \isEnd
%     \quad
%     \isType[\typeEnv'']{\psi}{x_{ij}@p_i}{S_{ij}}
%     \quad
%     \isType[\typeEnv]{\psi}{e_{ij}@p_i}{S_{ij}}
%     \quad
%     \typeEnv'\subseteq \typeEnv
%     \\
%     \widetilde D = p_1(\VEC{x_1}, \VEC{k_1}), \ldots, p_n(\VEC{x_n}, \VEC{k_n})
%     \quad
%     \widetilde E = p_1(\VEC{e_1}, \VEC{k_1}), \ldots, p_n(\VEC{e_n}, \VEC{k_n})
%     \end{array}
%     } 
%   {\isType[\typeEnv, X(\widetilde D) \colon (\typeEnv',\typeEnv'' ;
%          \stypeEnv')]{\psi}{ X(\VEC{E}) }{\stypeEnv}} 
%    \\
% & \text{Data Typing }  
% \\[\ruleskip] & 
%   \qquad   \qquad   \qquad   \qquad   \qquad  \inferenceg{TD1}{}{\isData[t@p]} 
%   \qquad
%   \inferenceg{TD2}{}{\isData[v@p]}
%   \\ &
%   \inferenceg{TOD1}{}{\isOptData[e@p]}
%   \quad
%   \inferenceg{TOD2}{\isData[v]}{\isOptData[\some{v}@p]}
%   \quad
%   \inferenceg{TOD3}{}{\isOptData[\none@p]}
% \\
% & \text{State Formation } (\isAState[\sigma]), \\
% & \qquad \qquad \qquad\inferenceg{TS1}{}{\isAState[\emptyset]}
%   \qquad \qquad
%   \inferenceg{TS2}{\isAState[\sigma]\quad
%   \sigma(\thread[A], k) = \emptyset \quad \Blue{ X} \in
%   dom(\signature)}{\sigma,(\thread[A], k, \Blue{ X}) \colon \stateP}
%     \\[\ruleskip] & \qquad \qquad 
%   \inferenceg{TS3}{\isAState[\sigma]\quad
%   (\thread[A], k, \Blue{ X}) \in \sigma \quad \Blue{ Y} \in
%   dom(\signature)}{\exchange{X}{Y}(\sigma(t,k)) \colon \stateP}
% \qquad 
%   \inferenceg{TS4}{
%   \isAState[\sigma]\quad 
%   \isAState[\delta] 
%   % \quad
%   % \delta \subseteq \sigma
%   }{\sigma \backslash \delta \colon \stateP}\\
% & \text{Formulae Formation }  (\isAFormula[\ltypeEnv]),\\
% & 
%   \qquad
%   \inferenceg{TF1}{}{\isAFormula[\true]}
%   \quad
%   \inferenceg{TF2}{}{\isAFormula[\thread \colon \ownerTP{k}{A}{X} ]}
%   \quad
%     \inferenceg{TF3}{\isAFormula[ \psi] \quad \isAFormula[ \psi']
%   \quad \circ \in \{\otimes, \oplus \}   }{\isAFormula[ \psi
%   \circ \psi'  ]}
% \\ &\qquad \qquad \qquad \qquad \qquad \qquad \qquad
%     \inferenceg{TF4}{\isAFormula[ \psi] \quad \isAState[\delta]
%   }{\isAFormula[ \psi \backslash \delta
%    ]}
% % \\ &
% % \inferenceg{TGstruct}
% %   {
% %   \chor \action{\killOp{\killAct}} \chor'
% %   \quad
% %   \killAct \neq \gamma
% %   }  {\comp{\chor}{\chor''}{t}{\gamma} \action{\killOp{\killAct}}
% %   \comp{\chor'}{\chor''}{t}{\gamma}} 
  \end{align*}
}
  \caption{\GCQ: Type checking rules (excerpt): Premises for
    \Did{Tsel} are the same as for \Did{Tbcast}, without $\optdatap$ premises }
  \label{fig:global:types:selected}
\end{figure*}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig-global-causality.tex <==
\begin{figure}[t]
{\scriptsize 
  \begin{align*}
&\quad 
\inferenceg{TGinit}
{ \qquad \qquad
  \begin{array}{c}
  \isIndex{a}{\serviceT GAB} \qquad \qquad \qquad
\widetilde{\thread_q} \not\in \typeEnv
     \\      \isType[\Gamma,\isInit{ \widetilde{\thread_p[A] },
     \widetilde{\thread_q\left(B\right)}, k}]{\psi , \isInit{
    \widetilde{\thread_p[A]}, \widetilde{\thread_q[B]},
    k}}{\chor}{\stypeEnv, k \colon G}  
  \end{array}
  }
{ \isType{\psi}{ \initA{\widetilde{\thread_p[A]}}{
    \widetilde{\thread_q[B]}}{a}{k} \pfx \chor } {\stypeEnv}} 
\\[\ruleskip] &
\inferenceg{TGbcast}
  { \begin{array}{c}
      \isIndex[\typeEnv]{ \thread_1} { \ownerT{k}{A} } 
      \quad
      \isIndex[\typeEnv]{ \thread_i} { \ownerT {k}{B_i} } 
      \quad 
      \isIndex{e@\thread_1}{S}
      \quad
      \psi = \psi' ,  \psi''
      \quad
     \isType[\typeEnv, \VEC{x_p@\thread_p[B_p]} \colon S]{\psi''
      , \psi'''}{\chor}{\stypeEnv, k
     \colon G }
      \\
      \typerule{\psi' ,\thread_1 \colon \ownerT{k}{A} \lolli \psi'''}{}{\psi'''}
      % \quad
      % \notEntails{\ownerT{k}{A} \lolli \psi'}
      % \quad
      % \typerule{\psi,\psi'}{}{\chor}
      \quad
      \psi''' =\left(
      \bigoplus_{J = min(q(\widetilde{\thread_p[B_p]})) } \left(
      \bigotimes_{\thread_i \in J} (\thread_i : \ownerT{k}{B_i})\right)\right)
      \quad
      t_i \in {\widetilde{t_p[B_p]}}
    \end{array}
     }
  {\isType{\psi}{
    \left( \bcastA{\thread_1[A]}{\VEC{\thread_p[B_p]:x_p}}{q}{e}{k} \right) \pfx \chor }{\stypeEnv, k \colon \left(
     \bcastT{A}{\VEC B}{S} \pfx G \right) }} 
\\[\ruleskip] &
\inferenceg{TGred}
  { \begin{array}{c}
      \isIndex[\typeEnv]{ \thread_i} { \ownerT{k}{A_i} } 
      \quad
      \isIndex[\typeEnv]{ \thread} { \ownerT{k}{B} } 
      \quad 
      \isIndex{e_i@\thread_i}{S}
      \quad
      \psi = \psi' , \psi''
      \quad
      \isType[\typeEnv, x@t \colon S]{\psi'' , \psi'''}{\chor}{\stypeEnv, k
      \colon G }     
     \\
      \typerule{\psi' , \bigoplus_{J =
      min(q(\widetilde{\thread_i[A_i]}))} \left( \bigotimes_{\thread_i
      \in J}\left( \thread_i \colon \ownerT{k}{A_i} \right)\lolli
      \psi''' \right) }{}{\psi'''}
      \quad
      \psi''' = \thread \colon \ownerT{k}{B}
      \quad
      t_i \in {\widetilde{t_p[B_p]}}
      % \quad 
      % \notEntails{\bigoplus_{J =
      % min(q(\widetilde{\thread_i[A_i]}))} \left( \bigotimes_{\thread_i
      % \in J}\left( \thread_i \colon \ownerT{k}{A_i} \right)\lolli
      % \psi' \right)}
    \end{array}
     } 
  {\isType{\psi,\psi''}{\left( \reduceA{\VEC{\thread_p[A_p].e_p}}{\thread[B]:x}{q}{k}{op} \right) \pfx \chor }{\stypeEnv, k \colon
 \left(     \bcastT{\VEC A}{B}{S} \pfx G\right) }} 
\\[\ruleskip] &
\inferenceg{TGsel}
  { 
     \begin{array}{c}
     \isIndex[\typeEnv]{ \thread_1} { \ownerT{k}{A} } 
     \quad
     \isIndex[\typeEnv]{ \thread_i} { \ownerT{k}{B_i} } 
     \quad 
     \isType{\psi'}{\chor}{\stypeEnv, k
     \colon G_h }
       \quad
      \typerule{\psi'', \thread_1 \colon \ownerT{k}{A} \lolli \psi' }{}{\psi'}
       \\
      % \notEntails{\ownerT{k}{A} \lolli \psi'}
      % \quad
      % \typerule{\psi,\psi'}{}{\chor}
      % \quad
      \psi' =\left(
      \bigoplus_{J = min(q(\widetilde{\thread_p[B_p]})) } \left(
      \bigotimes_{t_i \in J} (\thread_i \colon \ownerT{k}{B_i})\right)\right)
      \quad
      t_i \in {\widetilde{t_p[B_p]}}
     \quad
     h \in I
     \end{array}
     } 
  {\isType{\psi,\psi''}{ \left( \choiceA{\thread_1[A]}{\widetilde{\thread_p[B_p]}}{q}{k}{l_h} \right)
     \pfx \chor}{\stypeEnv, k \colon \branchT A{\VEC B}lG}} \\
    % & \qquad \qquad \qquad \qquad
    %   \inferenceg{TGcomp}
    %   { 
    %   \isType[\typeEnv, \kappa : \killT ]{\psi}{P}{\stypeEnv} 
    %   \quad
    %   \isType[\typeEnv, \kappa : \killT ]{\psi}{Q
    %   }{\stypeEnv >> \stypeEnv'} 
    %   % \quad 
    %   % \trueProp{t \ge 0} 
    %   } 
    %   {\isType{\psi}{\comp P{Q}{}\killAct}{\stypeEnv';\stypeEnv''}} 
    % \\
    & 
%       \inferenceg{TGseq}
%       {\isType{\psi}{ \chorAct }{\stypeEnv_1} 
%       \quad 
%       \isType{\psi}{ \chor }{\stypeEnv_2} 
%       \quad 
%       \stypeEnv_1 \# \stypeEnv_2} 
%       {\isType{\psi}{ \chorAct \pfx \chor }{\stypeEnv_1 , \stypeEnv_2}} 
\qquad \qquad
            \inferenceg{TGsum}
            { \isType{\psi}{ \chor }{\stypeEnv} \quad \isType{\psi'}{ \chor' }{\stypeEnv} } 
            {\isType{\psi \oplus \psi'}{ \chor + \chor'}{\stypeEnv}} 
\qquad
\inferenceg{TGres}
  { \isType[\Gamma, r:S]{\psi}{ \chor}{\stypeEnv}} 
  {\isType[\Gamma]{\psi}{ \new{r} \chor}{\stypeEnv}} 
\\[\ruleskip] & 
\inferenceg{TGcond}
  { \isType{\psi}{\chor_1}{\stypeEnv} \quad \isType{\chor_2}{\psi}{\stypeEnv} \quad \isProp{e@\thread} } 
  {\isType{\psi}{ \ifthenelsek {e@\thread} {\chor_1} {\chor_2}
    }{\stypeEnv}} 
\quad
\inferenceg{TGinact}
  { \isEnd} 
  {\isType{\psi}{ \INACT }{\stypeEnv}} 
% \qquad \quad
% \inferenceg{TGkill}
%   { \isIndex{\kappa}{\killT}} 
%   {\isType{\psi}{ \killOp{\kappa}}{\stypeEnv}} 
\\[\ruleskip] & \qquad 
\inferenceg{TGrec}
  { \begin{array}{l}
      \isType[\typeEnv, X(\VEC D) \colon
      (\typeEnv';\stypeEnv')]{\psi}{\chor}{\stypeEnv}
      \quad
      \isType[\typeEnv', X(\VEC D) \colon
      (\typeEnv';\stypeEnv')]{\psi}{\chor'}{\stypeEnv'}
      \\ \qquad 
      \widetilde D = p_1(\VEC{x_1}, \VEC{k_1}), \ldots, p_n(\VEC{x_n},
      \VEC{k_n})
      \quad
      \isShared[\typeEnv'] \subseteq \typeEnv
    \end{array}
    } 
  {\isType{\psi}{ \recA{X}{\VEC{D}}{\chor'}{\chor} }{\stypeEnv}} 
\\[\ruleskip] & \qquad 
\inferenceg{TGcall}
  { 
    \begin{array}{l}
      \quad
    \isEnd
    \quad
    \isType[\typeEnv'']{\psi}{x_{ij}@p_i}{S_{ij}}
    \quad
    \isType[\typeEnv]{\psi}{e_{ij}@p_i}{S_{ij}}
    \quad
    \typeEnv'\subseteq \typeEnv
    \\
    \widetilde D = p_1(\VEC{x_1}, \VEC{k_1}), \ldots, p_n(\VEC{x_n}, \VEC{k_n})
    \quad
    \widetilde E = p_1(\VEC{e_1}, \VEC{k_1}), \ldots, p_n(\VEC{e_n}, \VEC{k_n})
    \end{array}
    } 
  {\isType[\typeEnv, X(\widetilde D) \colon (\typeEnv',\typeEnv'' ;
         \stypeEnv')]{\psi}{ X(\VEC{E}) }{\stypeEnv}} 
% \\ &
% \inferenceg{TGstruct}
%   {
%   \chor \action{\killOp{\killAct}} \chor'
%   \quad
%   \killAct \neq \gamma
%   }  {\comp{\chor}{\chor''}{t}{\gamma} \action{\killOp{\killAct}}
%   \comp{\chor'}{\chor''}{t}{\gamma}} 
  \end{align*}
}
  \caption{\GCQ: Type checking - Global types}
  \label{fig:global:types}
\end{figure}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig-global-semantics-selected.tex <==
\begin{figure}[t]
{\footnotesize 
  \begin{align*}
    & 
      \inferenceg{Init}% {^G|Init}
      {
      \begin{array}{c}
        \chorAct =     \initA{ \VEC{\thread_r[A]\Blue{\{Y_r\}}}
        }{ \VEC{\thread_s[B]\Blue{\{Y_s\}}}}{a}{k}
        \quad
        \sigma' = [(\thread_i,k)  |-> \Blue{ Y_i} ]^{|\VEC{\thread_r}|+|\VEC{\thread_s}|}_{i=1}
        \quad
        \VEC{n} = \VEC{\thread_s}, \{k\}
        \quad
        \VEC{n} ~\#~ \VEC{m} 
      \end{array}
      }
    {     \new{\VEC {m}}  \conf{\sigma}{ \chorAct
    % \initA{ \VEC{\thread_r[A]\{Y_r\}}
    % }{ \VEC{\thread_s[B] \{Y_s\}}}{a}{k} 
    \pfx \chor
    }
      \action{% \initA{ \VEC{\thread_r[A]}
    % }{ \VEC{\thread_s[B]}}{a}{k}  
    \chorAct
    } 
      \new{\VEC{m},\VEC{n}}\conf{\updateState{\sigma'}}{\chor} }
\\[\ruleskip] &
\inferenceg{Bcast}% {^G|Bcast}
    {       
     \begin{array}{c}
       J \subseteq \VEC{\thread_r}
       \quad
       q(J)
       \quad
       \forall {\iset i{\{A\} \cup J}}: \Blue{ X_i} \subseteq
       \sigma(\thread_i, k) \land
       \sigma'(t_i, k) = \exchange{\Blue{ X_i}}{\Blue{ Y_i}}(\sigma(t_i,k))
       \\
       \evalOp{e@\thread_A}{ v }
       \quad 
       \forall {\iset {i}{\VEC{\thread_r}}}: \theta(x_{i}) =
       \left\{
       \begin{array}{l} 
         \some{v} \quad i \in J  \\
         \none \quad \text{otherwise}
       \end{array}
       \right.
     \end{array}
    } {
    \new{\VEC{m}}\conf{\sigma}{    \left(
    \bcastA{
    \thread_A[A]\Blue{\{X_A;Y_A\}}
    }{\VEC{\thread_r[B_r]\Blue{\{X_r;Y_r\}}:x_r}}{q}{e}{k} \right) \pfx \chor
    } 
    \action{
    \theta(\chorAct)
    }\ 
    \new{\VEC{m}}    \conf{\sigma[\sigma']}{\theta(\chor) }}
\\[\ruleskip] &
\inferenceg{RedD}% {^G|RedD}
       {
                \begin{array}{c}
                  \preduces{\conf{\sigma}{\chorAct \pfx
                  \chor}}{\xi}{\conf{\sigma'}{\chorAct' \pfx \chor}}
                  \qquad
                  \enoughOutputs {\chorAct'}{\false}{\theta}
                \end{array}
       } {
                   \new{\VEC{m}}\conf{\sigma}{\chorAct \pfx \chor\ }
               \action{\tau}\ 
                   \new{\VEC{m}}\conf{\sigma'}{\chorAct' \pfx \chor }}
\quad 
    \inferenceg{RedE}% {^G|RedE}
    {       
    \begin{array}{c}
      \preduces{\conf{\sigma}{\chorAct \pfx
      \chor}}{\xi}{\conf{\sigma'}{\chorAct' \pfx \chor}}
      \qquad
      \enoughOutputs {\chorAct'}{\true}{\theta}
    \end{array}
    } { 
    \new{\VEC{m}}\conf{\sigma}{\chorAct \pfx \chor}
    \action{\theta(\chorAct')} 
    \new{\VEC{m}}\conf{\sigma'}{\chor \subst{\mathsf{op}(\theta)}{x@\thread_{j+1}}}}
  \end{align*}
}
  \caption{SOS for \GCQ (excerpt): $\chorAct$ in
    $\Did{BCast}$, $\Did{RedD}$  and $\Did{RedE}$ % and $\Did{Sel}$ 
    is defined as in $\Did{Init}$.}
  \label{fig:global:semantics}
\end{figure}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig-swap-and-store.tex <==
\begin{figure}[t!]
{\scriptsize
\begin{subfigure}[b]{\linewidth}
  \begin{gather*}
    \frac{ % Disjoint interactions
      \threads{\chorAct} ~\#~       \threads{\chorAct'} 
    }{
      \chorAct \pfx (\chorAct' \pfx \chor) \swaps \chorAct' \pfx (\chorAct \pfx \chor)
    }
\qquad 
    \frac{\thread[A] \notin \threads{\chorAct}}{
      \ifthenelsek {e@\thread[A]} { \chorAct \pfx \chor_1}
      { \chorAct \pfx \chor_2} \swaps
      \chorAct \pfx\ifthenelsek {e@\thread[A]} { \chor_1} { \chor_2} }
\\
    \frac{
      \thread_1[A] \neq \thread_2[B]
    }{
      \ifthenelsek {e@\thread_1[A]} {(\ifthenelsek {e'@q} {\chor_1} {\chor_2})}
      {(\ifthenelsek {e'@\thread_2[B]} {\chor'_1} {\chor'_2})} \swaps
      \ifthenelsek {e'@\thread_2[B]} {(\ifthenelsek {e@\thread_1[A]} {\chor_1} {\chor'_1})} 
      {(\ifthenelsek {e@\thread_1[A]} {\chor_2} {\chor'_2})}}
  \end{gather*}
  \caption{Swap congruence relation, $\swaps$}
  \label{fig:swap-rel}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
\centering
  \begin{align*}
    \Rule{
    Y =
       \left\{
       \begin{array}{l} 
         X \quad (\thread, k, X ) \in \sigma  \\
         \emptyset \quad \text{otherwise}
       \end{array}
       \right. \ 
    } 
    {  \sigma(\thread, k) = Y} 
    \qquad
    \Rule{
    \sigma ~\#~ \sigma'
    } 
    {  \updateState{\sigma'} = \sigma , \sigma'} 
    \qquad
    \Rule{
    % dom(\sigma) \cap dom(\sigma') = \delta 
    % \quad 
    \delta = \{ (\thread, k, X) ~|~ (\thread, k, X) \in \sigma \land
    (\thread, k, Y) \in \sigma'\}
    } 
    {  \updateState{\sigma'} = (\sigma\backslash \delta), \sigma'}     
  \end{align*}
\caption{Store update rules}
\label{fig:store-update}
\end{subfigure}
}
\caption{Swap congruence \ref{fig:swap-rel}, and Store update rules \ref{fig:store-update}}
\end{figure}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> global-calculus-types.tex <==

\section{Type System}

We now present our type system which allows to specify protocols in
terms of global types, and check whether session behaviours in a
choreography respect them. 

 \begin{definition}[Global Types: syntax]\label{globalcalculustypes}\rm
{\small
  \begin{align*}
    &    S &&::=\  % \phantom{{}\mid{}}
                                            \boolT \mid \intT \mid
                  \stringT \mid \ldots &&
                                                                   \Did{sort}
    \\
    % & U &&::=\  S 
    %        % \mid G@A %Delegation is excluded in this work
    %        && \Did{values} \\
    & G && ::=\  \bcastT A{\VEC{B}}S \pfx G && \Did{bcast} \\
    & &&  \phantom{{} \mid =  } \mid\redT {\VEC{A}}BS \pfx G && \Did{red} \\
    & &&  \phantom{{} \mid =  } \mid \branchT A{\VEC B}lG && \Did{branch} \\
    & &&  \phantom{{} \mid =  } \mid \endT && \Did{end} \\
    & &&  \phantom{{} \mid =  } \mid \recT t \pfx G  && \Did{rec} \\
    & &&  \phantom{{} \mid =  } \mid \callT t  && \Did{call} \\
  \end{align*}
}
\end{definition}

The syntax of global types describes the flow of interactions one can
have in \GCQ. Sorts $\boolT, \intT, \stringT, \ldots$ describe basic
value types. Type $\commT ABU \pfx G$ dictates the presence of a
communication from role $A$ to role $B$ of a value $U$, followed by a
continuation of type $G$. In type $\branchT ABlG$, role $A$ can select
in label $l_i$ offered by role $B$, following with a continuation of
type $G_i$. The type $\endT$ indicates termination and is often
ommited. Finally, type  $\recT{ t} \pfx G$ indicates a recursive type with $\callT t$
as a type variable, and it binds the free occurrences of
$\callT t$ in G. We take an equi-recursive view of types, not
distinguishing between $\recT t \pfx G$ and its unfolding
$G\subst{\recT{t} \pfx G}{\callT t}$. Notice that the syntax of global
types presented here is a subset of the originally presented in
\cite{Carbone:2013:DMA:2429069.2429101,M13:phd} not considering delegation. The
labelled type transition relation $\ltransition{G}{\alpha}{G'}$
expresses the abstract execution of
protocols. Its definition is presented in \cite[Figs. 5 \& 6]{Carbone:2013:DMA:2429069.2429101}.

A type judgment is written as $\isType{\chor}{\Delta}$, where $\Gamma$
is an unrestricted environment and $\Delta$ is a linear
environment. We commonly refer to $\Gamma$ and $\Delta$ as \emph{service} and
\emph{session } environments, respectively. Its syntax is defined in
Figure \ref{fig:global:environments}.


\begin{figure}[ht]
  \begin{align*}
    &    \typeEnv &&::=\  % \phantom{{}\mid{}}
                                            \emptyset     && 
    & \stypeEnv ::=\ &&  \phantom{ \mid =  }\emptyset \mid \stypeEnv, k : G && \Did{session}\\
    & &&  \phantom{ \mid =  }\mid \typeEnv, a \colon \serviceT GAB && \Did{service}   \\ 
    & &&  \phantom{ \mid =  } \mid \typeEnv, x@p \colon S && \Did{variable} 
    \\
    & &&  \phantom{ \mid =  } \mid \typeEnv, X(\widetilde D) \colon (\typeEnv ;
         \stypeEnv) && \Did{definition} 
    \\   
    & &&  \phantom{ \mid =  } \mid \typeEnv, p: \ownerT kA &&
                                                              \Did{ownership} 
    \\   
    & &&  \phantom{ \mid =  } \mid \typeEnv, \kappa: \killT && \Did{compensation} 
  \end{align*}

\caption{Global Types: Typing environments}
\label{fig:global:environments}
\end{figure}

A typing $a \colon \serviceT GAB$ defines the global type of a service
channel $a$, where $\VEC A$ and $\VEC B$ represent the roles of the
active and service processes, respectively. The typing $x@p \colon S$
restricts the contents of variable $x$ in $p$ to objects of sort
$S$. An ownership typing $p: \ownerT kA$ asserts that $p$ behaves as
the role $A$ in session $k$. A compensation typing $\kappa : \killT$
simply asserts that $\kappa$ is a compensation signal. Finally, the
typing $X(\widetilde D) \colon (\Gamma ;
         \Delta)$ keeps track of the environments needed to type
         recursive procedures.


\input{fig-global-types}


Figure \ref{fig:global:types} introduce the typing rules for the
global calculus.
%
In rule $\Did{TGinit}$ the sequence of interactions started with an
\Did{Init} action is typed: each process in the term is given
ownership to the role declared for it in the created session $k$
through the function $\isInit{ \widetilde{\thread_p[A] }, k}$, which returns a set of
   ownership assignments $\{\thread_q : \ownerT kB \mid \thread_q[B]
   \in \widetilde{\thread_p[A]}\}$. The condition $\VEC{\thread_q}
   \notin \typeEnv$ ensures that service threads are fresh. 
%
The typing rules for communications are grouped into $\Did{TGbcast}$, 
$\Did{TGred}$ and $\Did{TGsel}$. In each of them we must check that
the communication performed by the threads involved at both the sender
and receivers own their respective roles in the communication over the 
session in use. This is ensured by checking that the type environment
contains the ownership typings $\thread_p: \ownerT kA$ and $\thread_i:
\ownerT k{B_i}$ ($\irange i2j$) for a broadcast operation, and similarly
for reduce and selection. In $\Did{TGbcast}$, we additionally check
that the type expression sent by the sender corresponds to the carried
sort $<.S.>$, and that the continuation is typed according to the
initial type environment $\typeEnv$ extended with the assignment of
type $S$ to the variables used by the receiver threads in $\thread_2,
\ldots, \thread_j$. 
%
Rule $\Did{TGred}$ behaves complementary, ensuring that
each of the expresssions used by the sender threads behave according
to the same sort $<.S.>$, and ensuring that the continuation is typed according to the
initial type environment $\typeEnv$ extended with the assignment of
type $S$ to the variable used by the receiver in the communication. 
%
Rule $\Did{TGsel}$ types labelled selections: A selection of a label
$l_h$ on session $k$ is well-typed if the label is in those allowed by
the protocol of session $k$ $(h \in I)$. The continuation must then
implement the selected continuation $G_h$ on session $k$.
%

Rule $\Did{TGcond}$ is the standard typing rule used to type
conditional blocks: we must check that the expression $e@\thread$  is
a proposition, and that each of the branches of the conditional are
typed according to the session environment $\stypeEnv$.
%
Rule $\Did{TGres}$ types name restriction in the standard way. Observe
that if $r$ is a process identifier, then restriction only affect
$\typeEnv$ since $\stypeEnv$ does not refer to processes.

 Rule $\Did{TGinact}$ types
   termination: $\INACT$ is well-typed under any unrestricted
   environment $\typeEnv$ and session environment $\stypeEnv$ if each
   session $k$ typed in $\typeEnv$ has a type $\endT$, meaning that it
   has been succesfully terminated. Predicate $\isEnd$ is
   formalized as $\{\true \mid \forall k : G \in \stypeEnv, G
   = \endT\}$ and $\false$ otherwise.

 Rule $\Did{TGcomp}$.
Rule $\Did{TGsum}$.
Rule $\Did{TGkill}$.
Rules $\Did{TGrec}$ and 
$\Did{TGcall}$ type recursive definitions and their calls. In rule
$\Did{TGrec}$, the definition body can use all the shared channels and
previously defined procedures that are in $\typeEnv$ (function $\isShared$
returns the set of shared channel and definition typings in
$\typeEnv$). Rule $\Did{TGcall}$ is standard, checking that all
the expressions used for invoking the procedure have the same types as
their procedure definitions.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

